Recurrent Video Deblurring with Blur-Invariant Motion Estimation and Pixel Volumes

For the success of video deblurring, it is essential to utilize information from neighboring frames. Most state-of-the-art video deblurring methods adopt motion compensation between video frames to aggregate information from multiple frames that can help deblur a target frame. However, the motion compensation methods adopted by previous deblurring methods are not blur-invariant, and consequently, their accuracy is limited for blurry frames with different blur amounts. To alleviate this problem, we propose two novel approaches to deblur videos by effectively aggregating information from multiple video frames. First, we present blur-invariant motion estimation learning to improve motion estimation accuracy between blurry frames. Second, for motion compensation, instead of aligning frames by warping with estimated motions, we use a pixel volume that contains candidate sharp pixels to resolve motion estimation errors. We combine these two processes to propose an effective recurrent video deblurring network that fully exploits deblurred previous frames. Experiments show that our method achieves the state-of-the-art performance both quantitatively and qualitatively compared to recent methods that use deep learning.

==> figures/tables/bi_architecture.tex <==
%!TEX root = ../main_supp.tex
\begin{table}%
\centering
\begin{tabularx}{\columnwidth}{@{}YYYYYYY@{}}
  \hline
  \multicolumn{2}{c}{\emph{layer type}(\#)}&size & stride & out & norm & act.\\
  \hline
  \hline

  \multicolumn{7}{c}{\textbf{Feature Transform Layers}}\\
  \hline
  \multicolumn{2}{c}{\emph{Input}} & \multicolumn{5}{c}{$V_{t-1}$}\\
  \Xhline{0.3\arrayrulewidth}
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 64    & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 64    & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 64    & \emph{BN} & \emph{relu} \\
  \Xhline{0.3\arrayrulewidth}
  \multicolumn{2}{c}{\emph{add1}} & \multicolumn{5}{c}{\emph{Conv}, \emph{Input}}\\
  \hline

  \multicolumn{2}{c}{\emph{Concat}} & \multicolumn{5}{c}{$I_{t-1}^b$, $I_{t}^b$, $I_{t+1}^b$}\\
  \Xhline{0.3\arrayrulewidth}
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 64    & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 64    & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 64    & \emph{BN} & \emph{relu} \\
  \Xhline{0.3\arrayrulewidth}
  \multicolumn{2}{c}{\emph{add2}} & \multicolumn{5}{c}{\emph{Conv}, \emph{Concat}}\\
  \hline
  \multicolumn{2}{c}{\emph{Concat}} & \multicolumn{5}{c}{\emph{add1}, \emph{add2}}\\

  \hline
  \hline

  \multicolumn{7}{c}{\textbf{Encoder}}\\
  \hline

  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 64 & - & - \\
  \multicolumn{2}{c}{\emph{BN}1\_1} & - & - & - & - & -\\
  \multicolumn{2}{c}{\emph{relu}} & -  & - & - & - & - \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (2, 2) & 64 & \emph{BN} & \emph{relu} \\

  \Xhline{0.3\arrayrulewidth}

  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$ & (1, 1) & 128 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$ & (1, 1) & 128 & - & \\
  \multicolumn{2}{c}{\emph{BN}2\_2} & - & - & - & - & \\
  \multicolumn{2}{c}{\emph{relu}} & - & - & - & - & \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$ & (2, 2) & 128 & \emph{BN} & \emph{relu} \\

  \Xhline{0.3\arrayrulewidth}

  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$ & (1, 1) & 128 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$ & (1, 1) & 128 & - & \\
  \multicolumn{2}{c}{\emph{BN}3\_2} & - & - & - & - & \\
  \multicolumn{2}{c}{\emph{relu}} & -  & - & - & - & \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$ & (2, 2) & 128 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$ & (2, 2) & 128 & \emph{BN} & \emph{relu} \\

  \Xhline{0.3\arrayrulewidth}

  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 512 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 512 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 512 & \emph{BN} & \emph{relu} \\

  \hline
  \multicolumn{7}{c}{\textbf{Decoder}}\\
  \hline
  \multicolumn{2}{c}{\emph{DeConv3}} & $3\times3$  & (2, 2) & 256 & \emph{BN} & - \\
  \multicolumn{2}{c}{\emph{add}} & \multicolumn{3}{c}{\emph{DeConv3}, \emph{BN}3\_2} & - & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 256 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 256 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 256 & \emph{BN} & \emph{relu} \\

  \Xhline{0.3\arrayrulewidth}

  \multicolumn{2}{c}{\emph{DeConv2}} & $3\times3$  & (2, 2) & 128 & \emph{BN} & - \\
  \multicolumn{2}{c}{\emph{add}} & \multicolumn{3}{c}{\emph{DeConv2}, \emph{BN}2\_2} & - & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 128 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 128 & \emph{BN} & \emph{relu} \\

  \Xhline{0.3\arrayrulewidth}

  \multicolumn{2}{c}{\emph{DeConv1}} & $3\times3$  & (2, 2) & 64 & \emph{BN} & - \\
  \multicolumn{2}{c}{\emph{add}} & \multicolumn{3}{c}{\emph{DeConv1}, \emph{BN}1\_1} & - & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 64 & \emph{BN} & \emph{relu} \\
  \multicolumn{2}{c}{\emph{Conv}} & $3\times3$  & (1, 1) & 3 & - & - \\

  \hline

\end{tabularx}
\caption{Architecture of proposed \emph{PVDNet}. \emph{BN} denotes the batch normalization layer~\cite{Ioffe:2015:BatchNorm}.}
\label{tbl:bi_architecture}
\end{table}


==> figures/tables/bi_table.tex <==
%!TEX root = main.tex


%%%--------------------------------------------------------------------------------
\begin{table*}[t]
\centering
\begin{tabular}{ |c||c|c|c|c|c| }
\hline
Model & All & Top 10\% per video  & Bottom 10\% per video & Top 10\% all & Bottom 10\% all\\
\hline \hline
BI shape preserving & 28.8771& 30.5383& 26.9238& 32.7131& 24.6051 \\
BI_tv & 28.9457& 30.5781& 27.1163& 32.7788& 24.7119 \\
BI& 28.7785& 30.5949 & 26.6392 & 32.7508 & 24.2890 \\
ss&28.2106 & 30.5681	 & 25.0650 &32.8110& 22.6729 \\
ss_bb& 27.9109& 30.5482& 24.3123& 32.8291& 22.0280 \\
TVL1& 28.196& 30.7302& 25.0829& 33.2342& 22.7749 \\
FlowNet2& 27.8525& 29.7476& 25.7856& 31.5846& 23.5381 \\

\hline
\end{tabular}
\caption{Preliminary test. All models are trained for 50,000 iterations (supp)}
%\vspace{-0.4cm}
\label{tbl:pre_table}
\end{table*}
%%%--------------------------------------------------------------------------------

==> figures/tables/bi_table_aee.tex <==
%!TEX root = ../main_supp.tex
%%%--------------------------------------------------------------------------------
\begin{table}[t]
\centering
\begin{tabular}{ @{}|@{\hspace*{1mm}}c||@{\hspace*{2mm}}c@{\hspace*{2mm}}c@{\hspace*{2mm}}c|@{} }
\hline
% Model & Sintel Clean & Sintel Final & KITTI 2012 & KITTI 2015 & Middlebury\\
% \multirow{2}{*}{Model} & Sintel& Sintel& KITTI& KITTI& Middle\\
% & Clean& Final & 2012& 2015& bury\\

\multirow{2}{*}{Model} & Sintel& KITTI & \multirow{2}{*}{Middlebury}\\
& Clean/Final & 2012/2015 & \\
\hline \hline
TVL1 &22.44 / 21.98&53.59 / 49.26&8.34 \\
\emph{FlowNet2}& \textbf{2.08} / \textbf{3.62}& \textbf{3.45} / 7.74& \textbf{0.45} \\
% FlowNet2$_{ss}$& 13.95 / 11.69 & 46.39 / 65.40 & 0.76 \\
BIMNet & 3.41 / 4.98 & 3.74 / \textbf{7.17}& 0.60 \\

\hline
\end{tabular}
\caption{Comparison of motion estimation performance on public benchmarks. We computed AEE (average endpoint error) between the optical flows estimated by each method and the ground-truths provided in the benchmarks.}
%\vspace{-0.4cm}
\label{tbl:bi_table_aee}
\end{table}
%%%-------------------------------------------------------------------------------- 

==> figures/tables/bi_table_ss.tex <==
%!TEX root = ../main_supp.tex
% %%%--------------------------------------------------------------------------------
% \begin{table}[t]
% \centering
% \begin{tabular}{ |c||cc| }
% \hline
% Model & PSNR (dB) & SSIM\\

% \hline \hline
% \emph{FlowNet2}$_{SS}$ &\textbf{28.2106}&\textbf{0.9085}\\
% \emph{FlowNet2}$_{SS, BB}$ & 27.9206 & 0.8795 \\
% \emph{FlowNet2}$_{SS, BB, SB, BS}$ & 27.8915 & 0.8742\\
% \hline
% \emph{liteFlowNet}$_{SS}$ &\textbf{27.9084}&\textbf{0.8926}\\
% \emph{liteFlowNet}$_{SS, BB}$ & 27.2416 & 0.8271 \\
% \emph{liteFlowNet}$_{SS, BB, SB, BS}$ & 27.2304 & 0.8207\\


% \hline
% \end{tabular}
% % \setlength{\abovecaptionskip}{5pt}
% % \setlength{\belowcaptionskip}{-10pt}
% \caption{Quantitative comparison of \emph{FlowNet} and \emph{liteFlowNet} trained with different combinations of input frames. We computed PSNR and SSIM between $I_{t}^s$ and $Warp(I_{t-1}^s, w^{bb})$. Errors were measured on the test set provided by Su~\Etal~\cite{su2017deep}.}
% \vspace{-0.4cm}
% \label{tbl:bi_table_ss}
% \end{table}
% %%%-------------------------------------------------------------------------------- 

%%%--------------------------------------------------------------------------------
\begin{table*}[t]
\centering
%\small
\begin{tabular}{ | c || c c | c c | c c | }
\hline
 \multirow{2}{*}{Model} & \multicolumn{2}{|c|}{Entire test set} & \multicolumn{2}{|c|}{Top 10\%} & \multicolumn{2}{|c|}{Bottom 10\%}\\
 & PSNR (dB) & SSIM & PSNR (dB) & SSIM & PSNR (dB) & SSIM\\
\hline \hline
\emph{FlowNet2}$_{SS}$                  & \textbf{28.21}  & \textbf{0.909} & 30.57           & 0.925          & \textbf{25.06}  & \textbf{0.811}\\
\emph{FlowNet2}$_{SS, BB}$              & 27.92           & 0.879          & 30.54           & 0.923          & 24.33           & 0.789\\
\emph{FlowNet2}$_{SS, BB, SB, BS}$      & 27.89           & 0.868          & 30.20           & 0.922          & 24.14           & 0.761\\
\emph{liteFlowNet}$_{SS}$               & 27.91           & 0.893          & 30.12           & 0.923          & 24.89           & 0.830\\
\emph{liteFlowNet}$_{SS, BB}$           & 27.41           & 0.821          & 30.05           & 0.907          & 24.12           & 0.778\\
\emph{liteFlowNet}$_{SS, BB, SB, BS}$   & 27.23           & 0.811          & 30.06           & 0.906          & 24.07           & 0.753\\

\hline
\end{tabular}
% \vspace{-0.1cm}
\caption{Quantitative comparison of \emph{FlowNet} and \emph{liteFlowNet} trained with different combinations of input frames. We computed PSNR and SSIM between $I_{t}^s$ and $Warp(I_{t-1}^s, w^{bb})$. Errors were measured on the test set provided by Su~\Etal~\cite{su2017deep}.}
\label{tbl:bl_table_ss}
\end{table*}
%%%--------------------------------------------------------------------------------

==> figures/tables/bi_table_ss_temp.tex <==
%!TEX root = ../main_supp.tex
%%%--------------------------------------------------------------------------------
\begin{table*}[h]
\centering
\begin{tabular}{ |c||cccccc| }
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Entire test set} & \multicolumn{2}{c}{Top 10\%}& \multicolumn{2}{c}{Bottom10\%}\vline \\ 
                       & \multicolumn{1}{l}{PSNR (dB)} & \multicolumn{1}{l}{SSIM}& \multicolumn{1}{l}{PSNR (dB)}& \multicolumn{1}{l}{SSIM}& \multicolumn{1}{l}{PSNR (dB)}& \multicolumn{1}{l}{SSIM}\vline \\

\hline \hline
TVL1 &\textbf{32.7802}&\textbf{0.9441 }&\textbf{33.2207}&\textbf{0.9471}&\textbf{32.3817}&\textbf{0.9421}\\
FlowNet2 & 29.4886 & 0.9231 &30.4927&0.9304&29.0997&0.9175 \\
MB-CLG & 19.3628 & 0.8035 &21.3870&0.8446&17.6935&0.7523 \\
FlowNet2$_{ss}$ & 30.6200 & 0.9259 &31.7381&0.9361&28.3345&0.8972 \\
BIMNet & 30.6795 & 0.9269 &31.4559&0.9345&29.8107&0.9147 \\


\hline
\end{tabular}
\caption{Quantitative comparison of motion estimation performance for blurry video frames. We computed average errors between $I_{t}^s$ and $Warp(I_{t-1}^s, w^{bb})$ in PSNR and SSIM, where $w^{bb}$ is the optical flow estimated from $I_{t}^b$ to $I_{t-1}^b$. Top 10\% and Bottom 10\% are test results for the most sharp and blurry 10\% frames per video, respectively.}
%\vspace{-0.4cm}
\label{tbl:bi_table_ss}
\end{table*}
%%%--------------------------------------------------------------------------------
